Conflict-based Search for Multi-Robot Motion Planning with Kinodynamic Constraints

Multi-robot motion planning (MRMP) is the fundamental problem of finding non-colliding trajectories for multiple robots acting in an environment, under kinodynamic constraints. Due to its complexity, existing algorithms either utilize simplifying assumptions or are incomplete. This work introduces kinodynamic conflict-based search (K-CBS), a decentralized (decoupled) MRMP algorithm that is general, scalable, and probabilistically complete. The algorithm takes inspiration from successful solutions to the discrete analogue of MRMP over finite graphs, known as multi-agent path finding (MAPF). Specifically, we adapt ideas from conflict-based search (CBS) - a popular decentralized MAPF algorithm - to the MRMP setting. The novelty in this adaptation is that we work directly in the continuous domain, without the need for discretization. In particular, the kinodynamic constraints are treated natively. K-CBS plans for each robot individually using a low-level planner and and grows a conflict tree to resolve collisions between robots by defining constraints for individual robots. The low-level planner can be any sampling-based, tree-search algorithm for kinodynamic robots, thus lifting existing planners for single robots to the multi-robot settings. We show that K-CBS inherits the (probabilistic) completeness of the low-level planner. We illustrate the generality and performance of K-CBS in several case studies and benchmarks.

==> K-CBS IROS 2022/Sections/Conclusion.tex <==

In this work, we introduced an MRMP algorithm that is both scalable and probabilitically complete and poses no simplifying assumptions on the problem.  It initially operates as a fully-decentralized method by individually planning for each robot and posing constraints as conflicts between the robots are encountered.  It is equipped with a merging procedure that allows it to merge the robots with entangled paths to a meta-robot.  By doing so, it is able to utilize full-information (centralized) planning for only those robots while still treating others individually, leading to strong performance in various environments and settings.  
One can extend this work in several directions, such as designing heuristics to further improve performance and an adaptive method of choosing a value for the merging parameter.


==> K-CBS IROS 2022/Sections/Experiments.tex <==
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[scale=0.26]{Figures/empty_space/full_solution.png}%
%         \caption{Open Env. ($10\times 10$)}%
%         \label{fig:envOpen}%
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[scale=0.26]{Figures/corridor_space/full_solution.png}%
%         \caption{Narrow Env. ($5\times 4$)}%
%         \label{fig:envNarrow}%
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[scale=0.26]{Figures/maze_space/full_solution.png}%
%         \caption{Cluttered Env. ($15\times 15$)}%
%         \label{fig:envCluttered}%
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[scale=0.26]{Figures/MAPF_space/full_solution.png}%
%         \caption{Large Env. ($33\times 33$)}%
%         \label{fig:envLarge}%
%     \end{subfigure}\hfill
%     \caption{MRMP benchmark environments. The initial states are shown with small circles and goal regions with large circles.}
%     \label{fig:envs}
% \end{figure*}


% \begin{figure}[t]
%     \centering
%     \begin{subfigure}{0.48\columnwidth}
%         \centering
%         \includegraphics[height=3.2cm]{Figures/empty_space/full_solution.png}%
%         \caption{Open Env. ($10\times 10$)}%
%         \label{fig:envOpen}%
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.48\columnwidth}
%         \centering
%         \includegraphics[height=3.2cm]{Figures/corridor_space/full_solution.png}%
%         \caption{Narrow Env. ($5\times 4$)}%
%         \label{fig:envNarrow}%
%     \end{subfigure}\hfill
    
%     \begin{subfigure}{0.48\columnwidth}
%         \centering
%         \includegraphics[height=3.2cm]{Figures/maze_space/full_solution.png}%
%         \caption{Cluttered Env. ($15\times 15$)}%
%         \label{fig:envCluttered}%
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.48\columnwidth}
%         \centering
%         \includegraphics[height=3.2cm]{Figures/MAPF_space/full_solution.png}%
%         \caption{Large Env. ($33\times 33$)}%
%         \label{fig:envLarge}%
%     \end{subfigure}\hfill
%     \caption{MRMP benchmark environments. The initial states are shown with small circles and goal regions with large circles.}
%     \label{fig:envs}
% \end{figure}


Here, we show the performance of \Alg{K-CBS} in four different environments 
(Open, Narrow, Cluttered, and Large) shown in Fig.~\ref{fig:envs}
with various numbers of robots, each with 2nd-order car dynamics (5-dimensional state space):
\begin{align*}
    \dot x= v \cos \theta, \; \dot y = v \sin \theta, \; \dot \theta = \frac{v}{l} \tan \phi, \;
    \dot v = u_1, \;  \dot \phi = u_2
\end{align*}
where $x$ and $y$ define the position, $\theta$ is the orientation, $v$ is the velocity, $\phi$ is the steering angle, $u_1$ is the acceleration rate and $u_2$ is the steering rate. 
%and the controls $u_1$ and $u_2$ are the acceleration and steering rate, respectively.  
Each robot has a rectangular shape with length $l=0.7$ and width $w=0.5$.

In each environment, we benchmarked the performance and scalability of \Alg{K-CBS} against two baseline approaches: centralized \Alg{RRT} (\Alg{cRRT}) and prioritized \Alg{RRT} (\Alg{pRRT})~\cite{lavalle2006planning}.\footnote{Comparison against  \cite{Le:ICAPS:2017,Le:RAL:2019} (without the PID controller) did not materialize due to unavailability of the code and complicacy
%\shtodo{changed from "complexity" to "complicacy", so not to confuse with computational complexity.}
of the algorithm.}  
\Alg{cRRT} is a centralized method that plans in the composite space of all the robots, whereas \Alg{pRRT} 
is a decentralized algorithm that plans for each robot $i$ in turn, treating the plans for robots $1, \ldots, i-1$ as timed obstacles.
%moving obstacles.% while planning for agent $i$.
We also varied the merging parameter $B$ to show its effect on the performance of \Alg{K-CBS}.
Every benchmark consisted of $100$ problem instances with a timeout of $5$ minutes. 
The comparison metrics are \emph{success rate}, \emph{computation time} (of successful runs), and \emph{merge rate}. 
The results are shown in Fig.~\ref{fig:bench_open}-\ref{fig:bench_cluttered} and Table~\ref{tab:benchmarkTable}.  

Our implementation of \Alg{K-CBS} utilized the classical RRT as the low-lever planner. The code is publicly available on GitHub~\cite{sourceCode}.
% \shtodo{removed the additional details, as they don't seem necessary.}
% Our implementation of \Alg{K-CBS} utilized the classical RRT as the low-lever planner.   
% Our code is publicly available on GitHub~\cite{sourceCode}, which uses the Open Motion Planning Library (OMPL) \cite{sucan2012the-open-motion-planning-library}.  
%We also implemented \Alg{cRRT} and \Alg{pRRT} in OMPL.
The benchmarks were performed on 
%the same machine with 
AMD Ryzen 7 3.9 GHz CPU and 64 GB of RAM.



\begin{figure*}%
    \centering
    % \begin{subfigure}{\textwidth}
        \includegraphics[width=.8\textwidth]{Figures/empty_space/ratio_6_1/success_rate.png}%
        % \caption{Success Rate}%
        % \label{fig:bench_empty_space_successRate}%
    % \end{subfigure}
    % \newline
    
    % \begin{subfigure}{\textwidth}
        \includegraphics[width=.8\textwidth]{Figures/empty_space/ratio_6_1/computation_times.png}%
        % \caption{Computation Times}%
        % \label{fig:bench_empty_space_compTime}%
    % \end{subfigure}\hfill%
    \caption{Benchmark results for the Open environment in Fig.~\ref{fig:envOpen} 
    % comparing \Alg{cRRT}, \Alg{pRRT}, and \Alg{K-CBS} with varying values of $B$.
    }
    \label{fig:bench_open}
\end{figure*}
\begin{figure*}%
\centering
    % \begin{subfigure}{0.9\columnwidth}
    \includegraphics[width=.32\textwidth]{Figures/corridor_space/success_rate.png}%
    % \caption{Success Rate}%
    % \label{fig:bench_corridor_space_successRate}%
    % \end{subfigure}\hfill
    % \begin{subfigure}{0.45\columnwidth}
    \hfill
    \includegraphics[width=.32\textwidth]{Figures/corridor_space/computation_times.png}%
    \hfill
    % \caption{Computation Times}%
    % \label{fig:bench_corridor_space_compTime}%
    % \end{subfigure}\newline%
    % \begin{subfigure}{0.45\columnwidth}
    \includegraphics[width=.32\textwidth]{Figures/corridor_space/merge_rate.png}%
    % \caption{Merge Rates}%
    % \label{fig:bench_corridor_space_mergeRates}%
    % \end{subfigure}\newline%
    \hfill
    \caption{Benchmarks of the Narrow environment in Fig.\ref{fig:envNarrow}
    % comparing \Alg{cRRT}, \Alg{pRRT}, and \Alg{K-CBS} with varying values of $B$.
    }
    \label{fig:bench_corridor}
\end{figure*}
\begin{figure*}
    \centering
    % \begin{subfigure}{\textwidth}
        \includegraphics[width=0.85\textwidth]{Figures/maze_space/ratio_6_1/success_rate.png}%
        % \caption{Success Rate}%
        % \label{fig:bench_corridor_maze_successRate}%
    % \end{subfigure}\newline
    
    % \begin{subfigure}{\textwidth}
        \includegraphics[width=.85\textwidth]{Figures/maze_space/ratio_6_1/computation_times.png}%
        % \caption{Computation Times}%
        % \label{fig:bench_corridor_maze_compTime}%
    % \end{subfigure}\newline%
    % \begin{subfigure}{\textwidth}
    % \centering
    % \includegraphics[width=\columnwidth]{Figures/maze_space/merge_rate.png}%
    % \caption{Merge Rates}%
    % \label{fig:bench_corridor_maze_mergeRates}%
    % \end{subfigure}\newline%
    \caption{Benchmark results for the Cluttered Env. in Fig.~\ref{fig:envCluttered}.}
    \label{fig:bench_cluttered}
    \vspace{-1mm}
\end{figure*}


\paragraph*{Open Environment}
In this environment, the robots have to swap positions, i.e., each robot starts in the center of the goal region of another robot (Fig.\ref{fig:envOpen}). We varied the number of robots from 2 to 6.  The results are shown in Fig.~\ref{fig:bench_open}. 
Note that \Alg{cRRT} is only able to find solutions for the two-robot case (10-dimensional composed state space) with a low success rate.  For larger number of robots, its success rate was zero (hence, not shown in Fig.~\ref{fig:bench_open}).  On the other hand \Alg{pRRT}, due to its decentralized nature, performs well in this environment with a success rate of 100\% for all cases.
However, as the number of robots increases, \Alg{pRRT} spends an increasingly large amount of time collision checking against prior robots during planning, resulting in long computation times.  \Alg{K-CBS} does not consider other agents until an entire plan is found. Thus, it scales much better than \Alg{pRRT} with 1--2 orders of magnitude smaller computation times, especially if $B$ is large. 
% generally 10-??? x faster computation times.  
Observe that for $B = 1$, \Alg{K-CBS} merges robots after one conflict, leading to planning in a larger dimensional space.  Clearly, in open environments such a hasty merge is inadvisable.

\paragraph*{Narrow Environment}
In this environment, the narrow corridors are only wide enough for a single robot to traverse at a given time (Fig.~\ref{fig:envNarrow}). Thus, the blue robot must remain out of the corridor until the green agent leaves it, at which point it may travel safely to goal. The benchmark results are shown in Fig.~\ref{fig:bench_corridor}. \Alg{pRRT} struggles in this space because there is no way to consider the blue and green agents simultaneously to ensure success. On the other hand, \Alg{cRRT}, which considers all three agents simultaneously, always fails due to the blow-up in the (15-dimensional) search space.  Conceptually, \Alg{K-CBS} 
%operates somewhere in the middle 
finds a balance in the middle
by merging the blue and green robots but not the red one. 
This leads to a high success rate in this space, 
%This enables it to be very successful in this space, 
particularly for low values of $B$, where the composed agents have the most time to traverse the narrow corridor.

\paragraph*{Cluttered Environment}
Here, we further consider the scalability of \Alg{K-CBS} against \Alg{pRRT} by analyzing it on a larger space with many obstacles and increasing the number of robots from 3 to 10 (Fig.~\ref{fig:envCluttered}). The results are shown in Fig.~\ref{fig:bench_cluttered}. Once again, we see that \Alg{pRRT} spends most of its time collision checking and does not scale past $7$ robots. For \Alg{K-CBS}, higher values of $B$ are more successful in all cases while also generating solutions faster than \Alg{pRRT}. 

\paragraph*{Large Environment}
The large environment, depicted in Fig.~\ref{fig:envLarge}, is used to test the limits of \Alg{K-CBS}. The results are in Table~\ref{tab:benchmarkTable}. \Alg{pRRT} failed on every instance, but \Alg{K-CBS} reliably scales up to $20$ agents. % when not merging at all ($B=\infty$).
% Indeed, in complex examples with open spaces, resolving constraints is less hindering than merging multiple pair of agents.
%it is quicker to resolve many constraints than to merge multiple pairs of agents. 

Overall, our benchmarks of \Alg{K-CBS} for many $B$-values and scenarios suggest that (i) \Alg{K-CBS} is scalable and (ii) merging is most useful in cases where agents must carefully coordinate their movement together in a small space (e.g., corridor).  In more open spaces, large values should be chosen for $B$ to avoid unnecessary merges.
%In general, merging should be avoided. Only in specific corner cases, such as agents bypassing each other in narrow corridors is merging beneficial. 
Still, \Alg{K-CBS} solves very complex MRMP instances reliably and quickly compared to current methods. 

\input{Sections/table}

% \jk{Hand-design examples added but I am sure if we like showing the full solutions as is. I have also included the solutions explanation and empty spaces with start and goal regions only in case that could look better.}
% \label{subsec:examples}




% \subsection{Benchmark Evaluation}


% \begin{figure}%
% \centering
%     % \begin{subfigure}{0.9\columnwidth}
%     \includegraphics[width=.8\columnwidth]{Figures/corridor_space/success_rate.png}%
    
%     % \caption{Success Rate}%
%     % \label{fig:bench_corridor_space_successRate}%
%     % \end{subfigure}\hfill
%     % \begin{subfigure}{0.45\columnwidth}
%     \includegraphics[width=.8\columnwidth]{Figures/corridor_space/computation_times.png}%
    
%     % \caption{Computation Times}%
%     % \label{fig:bench_corridor_space_compTime}%
%     % \end{subfigure}\newline%
%     % \begin{subfigure}{0.45\columnwidth}
    
%     \includegraphics[width=.8\columnwidth]{Figures/corridor_space/merge_rate.png}%
%     % \caption{Merge Rates}%
%     \label{fig:bench_corridor_space_mergeRates}%
%     % \end{subfigure}\newline%
%     \caption{Benchmarks of corridor space comparing \Alg{cRRT}, \Alg{pRRT}, and \Alg{K-CBS} with varying values of $B$.}
%     \label{fig:bench_corridor}
% \end{figure}


==> K-CBS IROS 2022/Sections/Introduction.tex <==


% \shtodo{Why did we change from Multi-agent to Multi-robot?}
% \ml{both MAMP and MRMP are apparently used in the community. We decided to go with MRMP since robots are known to have dynamical constraints but agents may not.  Not a strong preference though.}
% \shtodo{Ok. It clashes with the song :) But it's fine to leave it as robots.}

\textit{Multi-robot motion planning} (MRMP) is a fundamental challenge in robotics and artificial intelligence. The goal of MRMP is to compute dynamically-feasible trajectories for multiple robots to reach their respective goal regions such that, when executed simultaneously, the robots do not collide with obstacles nor with each other. MRMP has vast applications, from  warehouse robotics and delivery to planetary exploration and search-and-rescue.  
% of MRMP are found in numerous settings where multiple moving agents operate in a shared workspace.
The difficulty of MRMP lies in the size of the planning space, which grows exponentially with the number of robots.  In addition, there are constraints posed by the robots kinodynamics that need to be respected, which by itself is a difficult problem even for a single robot -- \textbf{NP-hard} for simple cases of a point robot with Newtonian dynamics \cite{DXPR93nphard} and curvature-constrained planar Dubins car (linear dynamics) \cite{kirkpatrick2011hardness}, and for nonlinear robots, the complexity is unknown (likely undecidable).
% \shtodo{This paper claims it's undecidable: https://www.sciencedirect.com/science/article/pii/030439759400147B 
% \\ I found this reference from a paper by Plaku.}
% \ml{I think that paper claims undecidability for hybrid systems.  I'm not sure if it holds for just nonlinear systems. we could cite it because we can consider/handle hybrid dynamics as well.}
% \shtodo{I see. I didn't realize this was open. Seems like an interesting problem.}
% and in general it is \textbf{PSPACE-hard} [64], meaning it is at least as hard as solving any \textbf{NP-complete} problem.
% There are two general approaches to MRMP: \emph{centralized} (coupled) and \emph{decentralized} (decoupled). The centralized methods \cite{solovey2015finding,wagner2015subdimensional,shome2020drrt} operate over the composed space of all the agents, and \emph{decentralized} approaches, divide the problem into several sub-problems and solve each separately \cite{gammell2014bit,sanchez2002using,van2005prioritized,tang2018complete}. 
% Centrazlized approaches have strong completeness and optimality properties, but they are not scalable.  Decetnralized approaches are scalable, but often do not provide any performance guarantees.  
For this reason, either simplifying assumptions are posed on the problem (e.g., removal of the dynamic constraints) or incomplete algorithms are accepted for the purposes of scalability.
In this work, without any simplifying assumptions, we aim to develop a scalable kinodynamic planner for MRMP with (probabilistic) completeness guarantees.


MRMP has been extensively studied in the robotics community.  
The approaches are generally classified into two categories: \emph{centralized} (coupled) and \emph{decentralized} (decoupled). 
% \cite{lavalle2006planning}\shtodo{Remove thisreference?}. 
The centralized methods (e.g., \cite{wagner2015subdimensional,shome2020drrt})
% \shtodo{Remove \cite{solovey2015finding}) 
operate over the composed state space of all the robots.   
The advantage of these approaches is that they allow the use of the rich library of existing single-robot motion planners (e.g., RRT \cite{Lavalle98rapidly-exploringrandom}
% , EST \cite{hsu1997path}, 
and KPIECE \cite{sucan2011sampling}) and automatically inherit their completeness and optimality.
%properties.  
The disadvantage is that they are not scalable.  
In contrast, 
%To address this issue, 
decentralized approaches divide the problem into several sub-problems and solve each separately \cite{gammell2014bit,sanchez2002using,van2005prioritized,tang2018complete}.
% Decentralized approaches, such as \ml{explain and cite P-RRT} are scalable, but often do not provide any performance guarantees.
While successful in scalability, 
% The major problem with the 
existing decentralized MRMP algorithms are mostly incomplete, i.e., do not guarantee to find a solution if one exists.

The discrete analogue of MRMP, dubbed \emph{multi-agent path finding} (MAPF), has received much attention in the AI and discrete planning community. There, the agents travel along edges in a discrete graph (rather than a continuous space).
%In the AI and discrete planning community, a similar problem to MRMP is considered over discrete graphs (rather than continuous space), known as the \emph{multi-agent path finding} (MAPF) problem.  
The main focus in MAPF is scalability, and as a result,  advanced algorithms have been developed that are not only scalable, but also have completeness and optimality guarantees (see \cite{stern2019mapf} and references therein). %\cite{stern2019mapf,standley2010finding,AFeln17c,AFeln16c,JSvan18b,SKoen18k,SKoen19a}. 
%\shtodo{I suggest replacing all of these by: (see \cite{stern2019mapf} and references therein).} 
A popular decentralized algorithm is \emph{conflict-based search} (CBS) \cite{SHARON201540}, which plans for each agent separately using low-level search (e.g., $A^*$). It then identifies collisions in the proposed plans and re-plans for colliding agents after placing path-constraints that resolve the collision. Thus, CBS grows a ``conflict tree'', where each node represents a (possibly colliding) plan.
%It uses a low-level search (e.g., $A^*$) to plan for a single agent at each iteration, and grows a constraint tree at the high level to identify and place constraints on the computed paths to avoid collision with other agents.  
%\shtodo{I think that for readers not familiar with MAPF/CBS, this will not be helpful. I can revise, if you agree.}
%\ml{yes, thanks!}

Unfortunately, such MAPF algorithms cannot be utilized to solve the MRMP problem in a straightforward manner, since MAPF abstracts the continuous workspace into a finite graph (e.g., a grid world),
and ignores the shape of the robots.  It also bypasses all dynamic constraints by assuming every edge of the graph is realizable with a known time duration. 
% but it in addition, to discrete space, the kinodynamical constraints are not possible to include.\\

Several works have focused on adapting MAPF algorithms to handle the challenges of MRMP, e.g.,
%addressing those challenges to be able to adopt MAPF algorithms for MRMP, e.g., 
\cite{solis2021representation, honig2018trajectory, Le:ICAPS:2017, Le:RAL:2019, WEN2022103997}.  
Work \cite{solis2021representation} combines continuous \emph{probabilistic roadmaps} (PRM) planner \cite{kavraki1996probabilistic}
with CBS to solve the robotics version of MAPF by ignoring the kinodynamic constraints.  Work \cite{honig2018trajectory}
accounts for dynamics and
uses CBS with optimization techniques for a swarm of quadrotors.  
Specifically, it first performs a discretization of the workspace (grid), and uses CBS to compute discrete paths.  Then, it uses an optimization formulation to generate controllers for the quadrotors to follow the discrete paths.  To guarantee correctness, it assumes sphere-shaped quadrotors with linear dynamics.
% \shtodo{multi-rotors? it appears twice in the paragraph above.}
% \ml{yes. fixed!}
% \shtodo{What? Shouldn't it be multi-robots?}
% \ml{no, it's multi-rotors (e.g., quad-copter)}
% \shtodo{But the ``multi'' is about the number of robots, no?. That is, they have multiple quad-copters, they don't plan for each rotor as a separate agent, do they?}
% \ml{I modified the text to clarify it.}
While performing well for specific robots, those approaches do not generalize to robots with nonlinear dynamics.

% \ml{Justin, add CL-CBS to the above paragraph.  Any other work?}
% \jk{Car Like CBS (CL-CBS) does not belong in this paragraph as they reduce their setting to an MAPF problem. I did add its citation to the MAPF paragraph. I do not know of any work that would fit into this paragraph.}

To deal with general nonlinear dynamics, a powerful approach is sampling-based, tree-based motion planning.  To this end, recent work 
\cite{Le:ICAPS:2017,Le:RAL:2019} combine discrete search with a sampling-based tree planner to solve the MRMP problem.  The algorithm first discretizes the composed configuration space of all the robots using PRM, and then uses a discrete planner to find a candidate high-level plan (guide). 
Then, a sampling-based motion tree is grown in the composed space to follow the sequence of regions in the guide. If unsuccessful, a different guide is computed. This process repeats until a valid trajectory is found.  
The work uses centralized discrete planner at the high-level and grows the motion tree in the composed configuration space. Hence, it is probabilistically complete (i.e., the probability of finding a solution tends to one as the planning time tends to infinity, if a solution exists), but it may be slow. To speed up the planner, a feedback PID controller is assumed to drive each robot from one discrete region in the guide to the next.  While fast planning times can be achieved using this method, the choice for the size of PRM (discretization) is unclear, and the assumption on the controller is limiting, as they do not always exist.  

In this work, we introduce a decentralized, scalable MRMP planner that treats the kinodynamic constraints of the robots natively with probabilistic completeness guarantees.  Unlike related work that directly adopt MAPF algorithms on a discretized version of the problem, we incorporate the ideas that make CBS successful into the continuous domain using a sampling-based method. 
Our algorithm, dubbed \emph{Kinodynamic CBS} (\Alg{K-CBS}), like CBS, uses a low-level search and maintains a conflict tree.  The low-level search can be any (kinodynamic) sampling-based tree planner (e.g., RRT and KPIECE).  In each iteration of the algorithm, a plan is computed for an individual robot given a set of constraints (obstacles).  Then, collisions between the robot trajectories is checked.  If one exists, time-dependent obstacles are defined as constraints in the constraint tree, and a new planning query is specified accordingly.  
To ensure probabilistic completeness, we introduce a \emph{merge} method, by which we merge robots whose plans often conflict, into a single meta-robot.
% which enables to identify the robots with entangled paths and treat them as a meta agent.
% As results, K-CBS becomes probabilistically complete if of the low-level planner is probabilistically complete.

% \ml{Need to see if the results support the following claim:}
% Inspired by recent variants of CBS \cite{boyarski2015icbs,felner2018adding,li2019disjoint,li2019improved}, we also present a \emph{bypass} heuristic, which reduces the size of the constraint tree by allowing the low-level planner to incorporate new constraints within the same planning instance, leading to further performance improvement.



% \shtodo{I think the paragraph below should come before the ``in this work'' above.}
% \ml{the paragraph above explains what this paper does... the paragraph below is supposed to be very explicit about the contributions. Normally it should be short, but in this paper, I thought it was important to elaborate on the contributions to make sure the reviewers don't discount the impact of the work even though the algorithm seems like a pretty simple extension.  I'm open to suggestions to do it better.}
% \shtodo{Got it. Sure.}
The main contribution of this work is a decentralized, probabilistically-complete MRMP algorithm that is capable of generating kinodynamically feasible plans efficiently.  
Our planner, \Alg{K-CBS}, naturally adapts CBS from MAPF to MRMP. 
% Our planner, K-CBS, is a natural extension of single-robot 
This lifts every off-the-shelf (kinodynamic) sampling-based, tree-based planner to the multi-robot setting and removes all the limitations (assumptions) of state-of-the-art MRMP planners. Specifically, \Alg{K-CBS} operates completely in the continuous state space of the agents, hence, it does not require discretization nor a feedback-control design. It easily works with arbitrary, possibly heterogeneous, nonlinear dynamical models, and is capable of solving very complex MRMP instances efficiently. 
We empirically show the efficacy of \Alg{K-CBS} in many case studies, highlighting our algorithm's generality and performance improvements.



% There are two general approaches to MRMP: \emph{centralized} methods, which operate over the composed space of all the agents \cite{solovey2015finding,wagner2015subdimensional,shome2020drrt}, and \emph{decentralized} approaches, which divide the problem into several sub-problems and solve each separately \cite{gammell2014bit,sanchez2002using,van2005prioritized,tang2018complete}. In general though, the MRMP problem is \textbf{NP-Complete} and, because of this, much of the research related to MRMP focuses on solving a sub-problem, multi-agent path finding (MAPF). 

% MAPF abstracts the continuous workspace into a finite and discrete graph (visualized as a grid world), ignores the shape of the agent by solely considering (non-)occupied cells, bypasses all dynamical constraints by assuming a discrete set of control symbols (e.g. up, down, left, right) for every agent, and further assumes that individual symbols are executed simultaneously at discrete time points. 

% The importance of MAPF has generated a significant body of work over the past decade~\cite{stern2019mapf,standley2010finding,AFeln17c,AFeln16c,JSvan18b,SKoen18k,SKoen19a}, dealing with various aspects of the problem and suggesting increasingly scalable solutions. 
% In particular, a well-performing algorithm for MAPF is \emph{Conflict-Based Search (CBS)}~\cite{SHARON201540}, which is based on a decentralized approach, and has extensions with various heuristics that further improve its performance~\cite{boyarski2015icbs,li2019disjoint,li2019improved,felner2018adding}. CBS plans for a single agent at each iteration, while placing constraints on the suggested plans, so as to avoid collisions (we elaborate on CBS in Section~\ref{sec:Methods}).

% The main contribution of this work is a decentralized, probabilistically complete, MRMP algorithm capable of generating kinodynamically feasible motion plans in real-time. Our algorithm, dubbed \emph{Kinodynamic CBS} (K-CBS), lifts many requirements that exist in the current state-of-the-art. Specifically, K-CBS operates completely in the continuous state space of all agents, samples from the entire control space of a particular dynamics model (i.e. no control symbols or PID controllers), easily works with arbitrary, possibly heterogeneous, dynamical models, and capable of solving very complex MRMP instances in real-time. K-CBS extends CBS for MAPF to create an efficient kinodynamic multi-agent motion planning algorithm. We empirically show the efficacy of K-CBS in many case-studies, highlighting our algorithms generality and performance improvements.


% \jk{
% \cite{solis2021representation} has an extensive related work section about MRMP/MAPF that might help with our intro. Need to add CL-MAPF~\cite{WEN2022103997} and talk about how it abstracts the car into control symbols -- only works for cars. Need to add all of Plaku's works~\cite{Le_Plaku_2017, 10.5555/3304652.3304757, le2018cooperative, 8637037, le2021multi} and note that their works report really good computation times but utilize a PID controller
% }
% \ml{Justin, add more related work as you see fit.  Also, no need to cite all four papers by Plaku if they're all the same.}

==> K-CBS IROS 2022/Sections/Methodology.tex <==
We now present our solution to Problem~\ref{prob}, which takes inspiration from CBS. To this end, we first describe CBS for MAPF and then introduce the necessary extensions to solve the MRMP problem. Finally, we introduce our algorithm, \emph{Kinodynamic} CBS (\Alg{K-CBS}). 

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/constraint_exp_v1.png}
%     \caption{A visual representation of a conflict, collision, and constraint. Multiple conflicts occur during a single collision between the orange and blue robots within time range $t\in[t_i, t_e]$. The set of conflicts results in a single constraint for each robot, which are reasoned about separately.}
%     \label{fig:constraint}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/constraint_exp_v1.png}
%     % \caption{A visual representation of a conflict, collision, and constraint. Multiple conflicts occur during a single collision between the orange and blue robots within time range $t\in[t_i, t_e]$. The set of conflicts results in a single constraint for each robot, which are reasoned about separately.}
%     \label{fig:constraint}
% \end{figure*}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_1.png}%
        \caption{Proposed plan}%
        \label{fig:demo_initial}%
    \end{subfigure}\hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_2.png}%
        \caption{Collision starts at $t_s$}%
        \label{fig:demo_conflict_ts}%
    \end{subfigure}\hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_3.png}%
        \caption{Collision ends at $t_e$}%
        \label{fig:democ_conflict_te}%
    \end{subfigure}\hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_4.png}%
        \caption{Constraint on blue agent}%
        \label{fig:democ_conflict_constraint}%
    \end{subfigure}\hfill
    \caption{A visual representation of a conflict, collision, and constraint. Multiple conflicts occur during a single collision between the orange and blue robots within time range $t\in[t_s, t_e]$. The set of conflicts results in a single constraint for each robot, which are reasoned about separately. Constraint on orange agent not shown.}
    \label{fig:constraint}
\end{figure*}




\subsection{Conflict-Based Search for MAPF}
CBS is a two-level search on the space of possible MAPF plans, 
%over a MAPF graph with a finite set of vertices $V$ and edges $E$, 
and consists of a high-level conflict-tree search and a low-level graph search. 
At the high-level, CBS keeps track of a \emph{constraint-tree}, in which each node represents a suggested plan, which might have collisions, referred to as \emph{conflicts}. Initially, a root node is obtained by using a low-level graph search algorithm, typically $A^*$, to find a path for each robot from start to goal, ignoring the other robots (hence the decentralized nature of the method).

At each iteration, CBS picks an unexplored node from the constraint-tree, based on some heuristic, and identifies the conflicts (namely collisions) in the node's corresponding plan.
%by simulating the paths and checking for collisions. 
%\shtodo{Maybe drop the ``by simulating...'}
Then, CBS attempts to resolve the conflicts by creating child nodes based on the conflicts, as follows: if robots $i$ and $j$ collide at time $t$ in vertex $v$ (deonted $\langle i, j, v, t \rangle$), then two children are created for the node, one with the constraint that robot $i$ cannot be in vertex $v$ at time $t$ (denoted $\langle i, v, t \rangle$), and the other dually for robot $j$. Then, in each child node, a low-level search is used to replan a path for the newly-constrained robot, given the set of constraints obtained thus far along the branch of the constraint tree.
% %The idea is to plan for each robot individually using low-level graph search, while the high-level constraint tree tracks conflicts (collisions) between the robots and defines constraints to resolve them. 
This process repeats until either a non-colliding plan is found, or no new nodes are created in the constraint tree, 
at which point CBS returns that there is no solution. 




\subsection{MRMP Constraints}
\label{subsec:MRMP Constraints}
% fig 1: show both constraints -- red constraint shown as time dependent (transparency?, 2 figures?) -- nice to have both images -- thinner edge of workspaces -- MR is not a heuristic -- if worth it, turn BP to subsection
CBS definitions of conflicts and constraints fail for MRMP because (i) robots do not occupy vertices, and (ii) robots could have unique bodies. Additionally, due to the continuous time nature of MRMP, collisions occur over time intervals rather than time points as in MAPF. Thus, formal definitions of collisions and constraints for MRMP are needed.
% A MRMP conflict occurs when two robots $i$ and $j$ are located at states $\mathbf{x}_i(t)$ and $\mathbf{x}_j(t)$, respectively, such that, when projecting $\mathbf{x}_i(t)$ and $\mathbf{x}_j(t)$ onto workspace $W$, $\mathcal{S}_i$ and $\mathcal{S}_j$ are not disjoint. 
% We denote a conflict as $\langle i, j, \mathcal{S}_i, \mathcal{S}_j, t \rangle$. 

Given two trajectories $T_i$ and $T_j$ for robots $i$ and $j$, respectively, recall that a \emph{collision} occurs between robots $i$ and $j$ at every time point that Condition~\ref{cond:robotColliision} is violated.  The duration of a collision is the \emph{continuous} time interval the two robots are in collision as they 
%continue to 
evolve along their respective trajectories,
%%%%%%%
and we define a \emph{conflict} to be $K=\langle i,j,[t_s,t_e]\rangle$, where $t_s$ and $t_e$ are the start and end time of this interval.
%%%%%%%
% Let $t_s^K$ and $t_f^K$ be the starting and end time 
% %point and final time point 
% of this interval, respectively (see Fig.~\ref{fig:constraint}). 
% A \emph{conflict} is then
% %Then, we define a \emph{conflict}
% \begin{equation}
%     K=\{\langle i, j, \mathcal{S}_i(T_i(t_r)), \mathcal{S}_j(T_j(t_r)), t_r \rangle\ :\ t_r\in [t_s^K,t_f^K]\},
%     \label{eqn:collision}
% \end{equation}
% to be the set of time points where Condition~\ref{cond:robotColliision} is violated in a continuous time interval. 
Note that there may be multiple conflicts between trajectories $T_i$ and $T_j$, in which case their time intervals are disjoint.

A conflict $K=\langle i,j,[t_s,t_e]\rangle$ is resolved by imposing a \emph{constraint} $\mathcal{C}$ on either robot $i$ or robot $j$. Intuitively, a constraint on robot $i$ 
% requires $\mathcal{S}_i(T_i(t_r))$ not to collide with $\mathcal{S}_j(T_j(t_r))$ for all $t_r\in[t_i^K, t_f^K]$.
requires 
%robot $i$ 
it to avoid colliding with robot $j$ for all $t_r\in[t_s, t_e]$ by viewing $\mathcal{S}_j(T_j(t_r))$ as a moving (time-dependent) obstacle. 
%%%%%%%%
Formally, the constraint on robot $i$ for conflict $K$ is $\mathcal{C}_i=\{\langle i, \mathcal{S}_j(T_j(t_r)), t_r \rangle\ :\ t_r\in [t_s,t_e]\}$
%%%%%%%
% Formally, the constraint on robot $i$ for conflict $K$
% %in \eqref{eqn:collision} is defined as
% is
% \begin{equation}
%     % \mathcal{C}_i =\bigcup_{t_r=t_i}^{t_f}\langle i, \mathcal{S}_j, t_r\rangle,
%     \mathcal{C}_i=\{\langle i, j, \mathcal{S}_j(T_j(t_r)), t_r \rangle\ :\ t_r\in [t_i^K,t_f^K]\},
%     \label{eqn:constraint}
% \end{equation}
% \shtodo{Same comment as above about union.}
%which requires $\mathcal{S}_i(T_i(t_r))$ to not intersect with $\mathcal{S}_j(T_j(t_r))$ for every $t_r\in[t_i^K,t_f^K]$. 
%The dual constraint $\mathcal{C}_j$ on robot $j$ for the same conflict $K$
% may
%r equires it to avoid robot $i$ in the time interval $[t_i^K,t_f^K]$. 
% Note that bodies $\mathcal{S}_i(T_i(t_r))$ and $\mathcal{S}_j(T_i(t_r))$ must only be checked against each other for a single value of $t_r$. A shape along a trajectory must not be disjoint with the entire time interval of the collision. 
Thus, $\mathcal{C}_i$ treats $\mathcal{S}_j(T_j(t_r))$ as a moving obstacle rather than a static one for the entire time duration of the conflict (see Fig.~\ref{fig:constraint}).  We dually define the constraint $\mathcal{C}_j$ for robot $j$.
%
This splitting is the crux of the performance of the approach.
% \shtodo{is it crucial? since we're doing merges, we can do whatever we want, as long as we eventually merge everybody.}
% \shtodo{crucial for performance}
% A shape along a trajectory must not be disjoint with the entire time interval of the collision. 

Next, we describe how to resolve a conflict by re-planning for an individual robot with the corresponding constraint.


\subsection{Single-Robot Planning under MRMP Constraints}



To (re-)plan for individual robots, we can use any existing sampling-based, tree-search algorithm (e.g. RRT) since they are efficient in finding kinodynamically feasible trajectories.
% Sampling-based tree-search algorithms (e.g. RRT) are efficient in finding kinodynamically feasible trajectories.
A generic form of such planner $\mathcal{X}$ begins by initializing a graph $G$ at the initial state. Then, for $N$ iterations, the algorithm samples a state $\mathbf{x}_{rand}$, extends the motion tree towards $\mathbf{x}_{rand}$ by sampling an input and integrating \eqref{eqn:dyn}, and adds the trajectory to the graph after verifying that it is collision free. The process continues until a trajectory from the initial state to the goal region is found, or $N$ iterations is reached. 

% Although these planners perform well for single-query, single-robot kinodynamic planning, they are incapable of guaranteeing satisfaction of a set of constraints defined in Section~\ref{subsec:MRMP Constraints}. Thus, we present \Alg{Constrained-$\mathcal{X}$} (\Alg{CSTR-$\mathcal{X}$}), an extension of planner $\mathcal{X}$ that is capable of finding trajectories that do not violate a set of constraints $\mathcal{C}$. 

Such planners perform well for single-query, single-robot kinodynamic planning, but off-the-shelf, they are unable to guarantee the satisfaction of a set of constraints as defined in %~\eqref{eqn:constraint}. %(Sec.~\ref{subsec:MRMP Constraints}).  
 Sec.~\ref{subsec:MRMP Constraints}.
To this end, we present \Alg{Constrained-$\mathcal{X}$} (\Alg{CSTR-$\mathcal{X}$}, shown in Alg.~\ref{alg:cstrX}), an extension of planner $\mathcal{X}$ 
%that is capable of 
for finding trajectories that do not violate a set of constraints $\mathcal{C}$. 

% Although these planners perform well for single-query, single-robot kinodynamic planning, they are incapable of guaranteeing satisfaction of a set of constraints defined in Section~\ref{subsec:MRMP Constraints}. Thus, we present \Alg{Constrained-$\mathcal{X}$} (\Alg{CSTR-$\mathcal{X}$}), an extension of planner $\mathcal{X}$ that is capable of finding trajectories that do not violate a set of constraints $\mathcal{C}$. 

% Sampling-based tree-search motion planners performs well for single-query, single-robot kinodynamic planning. However, given a set of $c$ constraints $\mathcal{C}^i=\{\mathcal{C}_i^1, \ldots, \mathcal{C}_i^c\}$ imposed on robot $i$ as per Section~\ref{subsec:MRMP Constraints}, Alg.~\ref{alg:plannerX} is incapable of guaranteeing that no constraints from $\mathcal{C}^i$ are violated because $\mathcal{C}^i$ is not considered in the planning loop. 

% random state $\mathbf{x}_{rand}$, and computes the nearest $\mathbf{x}\in V$ to $\mathbf{x}_{rand}$, denoted as $\mathbf{x}_{near}$. Then, the algorithm computes a new state $\mathbf{x}_{new}$ by sampling $\mathbf{u}\in U$ and propagating $f$ from $\mathbf{x}_{near}$ toward $\mathbf{x}_{rand}$ for some small time interval $\Delta t$ (Line~\ref{ln:extend}). 
% A generic form of such planner $\mathcal{X}$ is shown in Alg.~\ref{alg:plannerX}. The algorithm takes as input a state space $X$, input space $U$, a dynamical constraint $f$, goal region $X^G$, obstacle set $\mathcal{O}$, initial state $\mathbf{x}_0\in X$, and number of iterations $N$. The algorithm begins by initializing a graph $G$ (Line~\ref{ln:initG}). Then, for $N$ iterations, the algorithm samples a random state $\mathbf{x}_{rand}$, and computes the nearest $\mathbf{x}\in V$ to $\mathbf{x}_{rand}$, denoted as $\mathbf{x}_{near}$ (Line~\ref{ln:sample}). Then, the algorithm computes a new state $\mathbf{x}_{new}$ by sampling $\mathbf{u}\in U$ and propagating $f$ from $\mathbf{x}_{near}$ toward $\mathbf{x}_{rand}$ for some small time interval $\Delta t$ (Line~\ref{ln:extend}). If the new trajectory $\overrightarrow{\mathbf{x}_{near},\mathbf{x}_{new}}$ avoids obstacles (Line~\ref{ln:collCheck}), then it is added to the tree (Line~\ref{ln:add}) and $\mathbf{x}_{new}$ is checked to be inside $X^G$ (Line~\ref{ln:goalCheck}). This process repeats for a maximum of $N$ times, terminating early if a solution $T=\overrightarrow{\mathbf{x}_{0},\mathbf{x}_{new}}$ is found (Line~\ref{ln:retSol}). 



% Sampling-based tree-search motion planners performs well for single-query, single-robot kinodynamic planning. However, given a set of $c$ constraints $\mathcal{C}^i=\{\mathcal{C}_i^1, \ldots, \mathcal{C}_i^c\}$ imposed on robot $i$ as per Section~\ref{subsec:MRMP Constraints}, Alg.~\ref{alg:plannerX} is incapable of guaranteeing that no constraints from $\mathcal{C}^i$ are violated because $\mathcal{C}^i$ is not considered in the planning loop. 
% \shtodo{We should explain why it isn't capable.}
% Additionally, our CBS-based solution could require that multiple queries be called for a given planning instance. 
% \shtodo{I don't understand this sentence.}
% Thus, we present \Alg{Constrained-$\mathcal{X}$} (\Alg{CSTR-$\mathcal{X}$}), 
% % a generalized sampling-based tree search algorithm capable of finding dynamically feasible trajectories that respect a set of constraints $\mathcal{C}$. 
% an extension of planner $\mathcal{X}$ that is capable of finding trajectories that respect a set of constraints $\mathcal{C}$. 

\begin{algorithm}[b]
\KwIn{($X$, $U$, $f$, $X^G$, $\mathcal{O}$, $\mathbf{x}_0$, N, $\mathcal{C}$, $\mathcal{T}$)}
\KwOut{Collision free trajectory $T$ that respects $\mathcal{C}$}
\eIf{$\mathcal{T}$ is empty}
{
    $G=\{V\leftarrow x_0, E\leftarrow \emptyset\}$\label{ln:newG}\;
}
{
    $G=\mathcal{T}$\label{ln:growT}\;
}
 \For{N iterations}
 {
    $\mathbf{x}_{rand}, \mathbf{x}_{near}\leftarrow$ \Alg{sample}($X$, $G.V$)\label{ln:sampleCSTR}\;
    $\mathbf{x}_{new} \leftarrow$ \Alg{extend}($\mathbf{x}_{rand}$, $\mathbf{x}_{near}$, $U$, $f$)\label{ln:extendCSTR}\;
    \If{isValid($\overrightarrow{\mathbf{x}_{near},\mathbf{x}_{new}}$, $\mathcal{O}$, $\mathcal{C}$)\label{ln:collCheckCSTR}}
    {
        $V\leftarrow V\cup \{\mathbf{x}_{new}\}$;
        $E\leftarrow E \cup \{\overrightarrow{\mathbf{x}_{near},\mathbf{x}_{new}}\}$\label{ln:addCSTR}\;
        \If{$\mathbf{x}_{new} \in X^G$\label{ln:golCheckCSTR}}
        {
            \KwRet{$\overrightarrow{\mathbf{x}_{0},\mathbf{x}_{new}}$\label{ln:retSolCSTR}}            
        }
    }
 }
\KwRet{$G(V,E)$ and ${\mathcal C}_{\max}$}
\caption{Constrained-$\mathcal{X}$ (CSTR-$\mathcal{X}$)}
\label{alg:cstrX}
\end{algorithm}

\Alg{CSTR-$\mathcal{X}$} 
%is shown in Alg.~\ref{alg:cstrX}, which 
takes two additional inputs than $\mathcal{X}$: a set of constraints $\mathcal{C}$, and an existing graph (motion tree) $\mathcal{T}$.
% \shtodo{I'm not sure if ``respects'' is clear enough. It certainly wasn't defined.}
% If $\mathcal{T}$ is non-empty, \Alg{CSTR-$\mathcal{X}$} utilizes the existing graph (Line~\ref{ln:growT}). Otherwise, it initializes a new graph $G$ with a single initial state $\mathbf{x}_0$ (Line~\ref{ln:newG}). The sample, select, and propagate procedures are identical to Planner $\mathcal{X}$ (Lines~\ref{ln:sampleCSTR}-\ref{ln:extendCSTR}). However, when checking a trajectory for validity (Line~\ref{ln:collCheckCSTR}), \Alg{CSTR-$\mathcal{C}$} checks against obstacles \emph{and} the constraint set $\mathcal{C}$.
If $\mathcal{T}$ is non-empty, \Alg{CSTR-$\mathcal{X}$} utilizes the existing graph (Line~\ref{ln:growT}). Otherwise, it initializes a new graph $G$ with a single initial state $\mathbf{x}_0$ (Line~\ref{ln:newG}). Then, to check if a trajectory is valid, \Alg{CSTR-$\mathcal{X}$} checks against both static obstacles $\mathcal{O}$ and constraints (moving obstacles) in $\mathcal{C}$ (Line~\ref{ln:collCheckCSTR}). 
Similar to existing validity checking functions, checking against $\mathcal{C}$ can be done efficiently, e.g., by discretizing the continuous trajectory $\overrightarrow{\mathbf{x}_{near},\mathbf{x}_{new}}$ into a set of points $\{x(\tau_1), \ldots, x(\tau_L)\}$ by sampling time at a fine resolution $\Delta t$, and checking $\mathcal{S}(\mathbf{x}(\tau_l))$ against all $\mathcal{C}^r\in \mathcal{C}$ for all $1\leq l \leq L$ such that $\tau_l$ is the time range of $\mathcal{C}^r$, i.e., $\tau_l \in [t^r_s, t^r_e]$.

The output of \Alg{CSTR-$\mathcal{X}$} is a trajectory that respects all the constraints, if one is found in $N$ iterations; otherwise, it returns the full motion tree, as well as the constraint ${\mathcal C}_{\max}$ that was violated the most.  Our \Alg{K-CBS} algorithm uses the motion tree to continue planning when needed, and uses ${\mathcal C}_{\max}$ to identify tangled plans, as discussed below.
Note that \Alg{CSTR-$\mathcal{X}$} defaults to Planner \Alg{$\mathcal{X}$} if both additional parameters $\mathcal{T}$ and $\mathcal{C}$ are empty sets.  

% Similar to existing collision checking function, checking against $\mathcal{C}$ can be done efficiently by dividing the continuous trajectory $\overrightarrow{\mathbf{x}_{near},\mathbf{x}_{new}}$ into a finite set of discrete states by only considering states at $\Delta t$ intervals. Then, for every state $\mathbf{x}(t)$ in that set, project $\mathbf{x}(t)$ onto the workspace $W$ to get shape $\mathcal{S}$ and evaluate it against all $\mathcal{C}^r\in \mathcal{C}$ such that $t\in [t_i, t_f]^r$ where $[t_i, t_f]^r$ is the time range of $\mathcal{C}^r$.

% \Alg{CSTR-$\mathcal{X}$} can be plugged onto any sampling-based tree search algorithm $\mathcal{X}$ to plan kinodynamically feasible trajectories that respect a set of time-dependent constraints of the form defined in \eqref{eqn:constraint}. Note that, if both additional parameters $\mathcal{T}$ and $\mathcal{C}$ are empty sets, \Alg{CSTR-$\mathcal{X}$} defaults to Planner \Alg{$\mathcal{X}$}. 
% These capabilities make \Alg{CSTR-$\mathcal{X}$} a great choice of low-level search for our algorithm, \emph{Kinodynamic} CBS. 
% \shtodo{I think the last sentence can be removed (also, I wouldn't use ``great'' at any point in the paper).}

% $\{(X_i, U_i, f_i, S_i, \mathbf{x}_{i,0}, X_i^G)\}_{i=1}^k$
\subsection{Kinodynamic Conflict-Based Search (\Alg{K-CBS})}
\begin{algorithm}[!ht]
\KwIn{$\{\mathcal{M}_i\}_{i=1}^{k}$, N, B}
\KwOut{Collision-free trajectories $\{T_1, \ldots, T_k\}$}
$Q, n_0, p_0, \leftarrow \emptyset$\;\label{ln:initKCBS}
\For{every robot $i$\label{ln:foreveryrobot}}
{
    $p_0 \leftarrow p_0 \cup$ \Alg{CSTR-X}($\mathcal{M}_i$, $\mathcal{O}$, $\mathbf{x}_{i,0}$, $\infty$, $\emptyset$, $\emptyset$)\label{ln:planInit}
    % \ml{shouldn't $\infty$ be $N$?}
    \;
}
$n_0$.plan $\leftarrow$ $p_0$; $Q$.\Alg{add}($n_0$) \label{ln:rootNode}\;
% \For{R iterations\label{ln:mainBegin}}
\While{solution not found \label{ln:mainBegin}}
{
    $c \leftarrow$ $Q$.\Alg{top}()\label{ln:selectKCBS}\;
    \eIf{$c$.plan is empty \label{ln:retry}}
    {
        $Q$.\Alg{pop}(); $\mathcal{C}^i \leftarrow$ $c.\mathcal{C}$; $\mathcal{T}^i \leftarrow$ $c.\mathcal{T}$\label{ln:retrySetup}\;
        $T_i',\mathcal{C}_{\max} \leftarrow$ \Alg{CSTR-X}($\mathcal{M}_i$, $\mathcal{O}$, $\mathbf{x}_{i,0}$, N, $\mathcal{T}^i$, $\mathcal{C}^i$)\label{ln:endRetry}\;
        \eIf{$T_i'$ is a trajectory}
        {
            $(c$.plan$\setminus T_i) \cup T_i'$\label{ln:retrySuc}\;
        }
        {
            $c$.tree $\leftarrow T_i'$ \label{ln:retryFail}\; 
            \If{\Alg{shouldMerge}($\mathcal{C}_{\max}$, B)\label{ln:mergeIf1}}
             {
                $\{\mathcal{M}_i\}_{i=1}^{k-1}\leftarrow$ \Alg{merge}($\{\mathcal{M}_i\}_{i=1}^{k}$,$\mathcal{C}_{\max}$)\label{ln:merge1}\;
                 $P\leftarrow$\Alg{K-CBS}($\{\mathcal{M}_i\}_{i=1}^{k-1}$, N, $B$)\;
                 \KwRet{$P$ \label{ln:mergeIf2}}
             }
        }
        $Q$.\Alg{add}($c$)\label{ln:retryAdd}\;
    }
    {
        K $\leftarrow$ \Alg{validatePlan}($c$.plan)\label{ln:validate}\;
        \uIf{K is empty\label{ln:isKempty}}
        {
            \KwRet{$c$.plan\label{ln:retPlan}}
        }
        \uElseIf{\Alg{shouldMerge}(K, B)\label{ln:shouldMerge}}
        {
            $\{\mathcal{M}_i\}_{i=1}^{k-1}\leftarrow$ \Alg{merge}($\{\mathcal{M}_i\}_{i=1}^{k}$, $K$)\label{ln:merge}\;
            $P\leftarrow$\Alg{K-CBS}($\{\mathcal{M}_i\}_{i=1}^{k-1}$, N, $B$)\label{ln:solveMeta}\label{ln:planMeta}\;
            \KwRet{$P$}
        }
        \Else{
            $Q$.\Alg{pop}()\label{ln:branchPop}\;
            \For{every robot $i$ in K\label{ln:branchForLoop}}
            {
                $\mathcal{C}^i \leftarrow$ $c.\mathcal{C} \; \cup$ K.\Alg{getCSTR}($i$); $c_{new} \leftarrow \emptyset$\label{ln:branchSet-up}\;
                $T_i' \leftarrow$ \Alg{CSTR-X}($\mathcal{M}_i$, $\mathcal{O}$, $\mathbf{x}_{i,0}$, N, $\emptyset$, $\mathcal{C}^i$)\label{ln:branchReplan}\;
                \eIf{$T_i'$ is a trajectory}
                {
                    $c_{new}\leftarrow(c$.plan$\setminus T_i) \cup T_i'$\label{ln:banchSuc}\; 
                    % $c_{new}$cost $\leftarrow c_{new}$.\Alg{getCost}()\;
                }
                {
                    $c_{new}$.tree $\leftarrow T_i'$\label{ln:branchFail}\; 
                }
            $Q$.\Alg{add}($c_{new}$)\label{ln:branchAdd}\;   
            }
        }
    }
    \label{ln:mainEnd}
}
\caption{Kinodynamic-CBS (K-CBS)}
\label{alg:K-CBS}
\end{algorithm}
% \jk{To Do: add labels to alg and reference in text.}
We now introduce the high-level algorithm of \Alg{K-CBS} (Alg.~\ref{alg:K-CBS}). %which is outlined in Alg.~\ref{alg:K-CBS}. 
Recall that the input to Problem~\ref{prob} comprises a state space $X_i$, input space $U_i$, vector field $f_i$, body $\mathcal{S}_i$, initial state $\mathbf{x}_{i,0}$, and goal region $X_i^G$ for every robot $i\in\{1, \ldots, k\}$. For brevity, we define a model $\mathcal{M}_i=\{X_i, U_i, f_i, \mathbf{x}_{i,0}, X_i^G\}$ as the inputs pertaining to robot $i$. The input to \Alg{K-CBS} is then a model for every robot $\{\mathcal{M}_i\}_{i=1}^{k}$, 
%a parameter $R$ of the maximum number of iterations of \Alg{K-CBS}, 
% \shtodo{what does ``iterations of the constraint tree'' mean?}
a parameter $N$ of the maximum number of iterations of \Alg{CSTR-$\mathcal{X}$}, and a merging parameter $B$. The output of \Alg{K-CBS} is a set of trajectories $\{T_1, \ldots, T_k\}$ 
% such that all trajectories are collision-free when executed simultaneously.
that is the solution to the MRMP problem.

\Alg{K-CBS} begins by calculating trajectories for every robot individually by calling \Alg{CSTR-$\mathcal{X}$} with an empty initial tree and empty set of constraints. These trajectories serve as the initial plan for the root node of the constraint-tree, which is added to a priority-queue $Q$ (Lines~\ref{ln:initKCBS}-~\ref{ln:rootNode}). 
The cost of node $n\in Q$ is the sum of control durations over all trajectories in the plan of $n$ (and $\infty$ if $n$ does not contain a plan yet). The smaller the cost of $n$, the higher its priority in $Q$.

At every iteration of \Alg{K-CBS}, a node $c \in Q$ with minimal cost is selected (Line~\ref{ln:selectKCBS}). If $c$ has a plan, it is evaluated for conflicts (Line~\ref{ln:validate}). If no conflict exists, then the plan is returned as the solution. 
Otherwise, an arbitrary conflict $K$ is selected and for each robot in $K$, and a constraint is generated.
%Otherwise every robots involved with a conflict is given a constraint and
Then, \Alg{CSTR-$\mathcal{X}$} is called to calculate a valid trajectory, storing the result of the search in a new node, which is added to $Q$ (Lines~\ref{ln:branchPop}-~\ref{ln:branchAdd}). If $c$ has no plan, another call to \Alg{CSTR-$\mathcal{X}$} is performed in an attempt to obtain such a plan (Lines~\ref{ln:retry}-~\ref{ln:retryAdd}). 

As \Alg{K-CBS} explores the space of all plans, it is possible that many conflicts are found between a particular pair of robots.  This can indicate that their motions are ``coupled,'' and hence, it is difficult to plan for them separately. In that case, \Alg{K-CBS} can merge the pair into a meta-robot and plan for an MRMP problem with $k-1$ robots %, where one robot is a meta-robot
(Lines~\ref{ln:mergeIf1}--\ref{ln:mergeIf2} and~\ref{ln:shouldMerge}--\ref{ln:planMeta}). We elaborate on this process below.
% in Section~\ref{subsec:MR}.

% \shtodo{Do we need a line-by-line breakdown of the algorithm? Isn't it better to explain what it does more intuitively? I think we're too short on space for the current explanation.}
% \ml{I agree... we need an intuitive explanation. The line-by-line description is hard to read.}
% \Alg{K-CBS} begins by initializing a priority queue $Q$ biased by some heuristic, initial constraint node $n_0$, and initial plan $p_0$ (Line~\ref{ln:initKCBS}). Next, $p_0$ is filled with a trajectory for every robot by calling \Alg{CSTR-$\mathcal{X}$} on every robot with an empty set of constraints and no existing tree (Line~\ref{ln:planInit}). Then, $p_0$ is saved in $n_0$, and then $n_0$ is added to $Q$ (Line~\ref{ln:rootNode}). From there \Alg{K-CBS} begins its main loop (Lines~\ref{ln:mainBegin}-~\ref{ln:mainEnd}) which can be divided into three main routines: \emph{branching}, \emph{retrying}, and \emph{merging}. We describe \emph{branching} and \emph{retrying} now but defer the explanation of \emph{merging} to Section~\ref{subsec:MR}. 

% At each iteration of \Alg{K-CBS}, the best unexplored constraint node in $Q$ is selected (Line~\ref{ln:selectKCBS}). In the first iteration, the selected node is $n_0$. Since $n_0$ has a plan, it is validated for conflicts (Line~\ref{ln:validate}). If no conflicts exist, the plan is returned as the solution (Lines~\ref{ln:isKempty}-~\ref{ln:retPlan}). Otherwise, \Alg{K-CBS} begins the branching procedure (Lines~\ref{ln:branchForLoop}-~\ref{ln:branchAdd}).

% The goal of branching is to resolve the conflict $K$. This is done by removing $c$ from $Q$ (Line~\ref{ln:branchPop}) and extending the constraint tree from $n_0$ for each robot in $K$ (Line~\ref{ln:branchForLoop}). First, robot $i$ in $K$ is given an additional constraint, the updated set of constraints $\mathcal{C}^i$ are gathered, and the new child constraint node is initiated (Line~\ref{ln:branchSet-up}). Next, \Alg{CSTR-$\mathcal{X}$} attempts to calculate a trajectory that respects $\mathcal{C^i}$ within $N$ iterations (Line~\ref{ln:branchReplan}). If successful, the new plan is saved in the new node $c_{new}$ by replacing the re-planed trajectory (Line~\ref{ln:banchSuc}). Otherwise, $c_{new}$ is not given a plan but it saves the tree from \Alg{CSTR-$\mathcal{X}$} (Line~\ref{ln:branchFail}). Either way, the nex node is added to $Q$ (Line~\ref{ln:branchAdd}).

% At the next iteration, the selected node $c$ could have a plan or not, depending on the outcomes of the re-planning call to \Alg{CSTR-$\mathcal{X}$} from the branching procedure. If $c$ has a plan, it is evaluated and possibly branched from again. If $c$, however, does not have a plan, then we must attempt to find one using the \emph{retrying} routine (Lines~\ref{ln:retry}-~\ref{ln:retryAdd}). 

% The routine begins by removing $c$ from $Q$, and gathering the saved set of constraints $\mathcal{C}^i$ and saved tree $\mathcal{T}^i$ (Line~\ref{ln:retrySetup}). Then, \Alg{CSTR-$\mathcal{X}$} attempts to find a trajectory that respects $\mathcal{C}^i$, this time, beginning with the tree $\mathcal{T}^i$ rather than from an empty one. Once again, if the planning query is successful, the plan is saved (Line~\ref{ln:retrySuc}). Otherwise, the updated tree is saved (Line~\ref{ln:retryFail}). Either way, the node is added back into $Q$ (Line~\ref{ln:retryAdd}).

% The branching and retrying routines continue until a collision-free plan is found. However, there are cases where creating a constraint eliminates the possibility of finding a valid plan. Therefore, we need a \emph{merging} routine that allows \Alg{K-CBS} to maintain completeness. 


\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.28]{Figures/incomplete_2.png}
    \caption{K-CBS tree. Robots must cross a narrow corridor.}
    \label{fig:incomplete}
\end{figure}



\begin{figure*}
    \centering
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[scale=0.26]{Figures/empty_space/full_solution.png}%
        \caption{Open Env. ($10\times 10$)}%
        \label{fig:envOpen}%
    \end{subfigure}\hfill
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[scale=0.26]{Figures/corridor_space/full_solution.png}%
        \caption{Narrow Env. ($5\times 4$)}%
        \label{fig:envNarrow}%
    \end{subfigure}\hfill
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[scale=0.26]{Figures/maze_space/full_solution.png}%
        \caption{Cluttered Env. ($15\times 15$)}%
        \label{fig:envCluttered}%
    \end{subfigure}\hfill
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[scale=0.26]{Figures/MAPF_space/full_solution.png}%
        \caption{Large Env. ($33\times 33$)}%
        \label{fig:envLarge}%
    \end{subfigure}\hfill
    \caption{MRMP benchmark environments. The initial states are shown with small circles and goal regions with large circles.}
    \label{fig:envs}
\end{figure*}

\subsubsection*{Merge and Restart}
\label{subsec:MR}
To clarify the concept of ``coupled'' robots,
consider the example 
%shown 
in Fig.~\ref{fig:incomplete}, where two robots must cross a narrow corridor that is just wide enough for the both of them. Assume that both robots have constant velocity toward their respective target and they only control their steering angle. When presenting \Alg{K-CBS} with this problem instance, the root node of the constraint tree could look like the one seen in at the top of Fig.~\ref{fig:incomplete}. Naturally, since both robots attempt to traverse through the middle of the corridor, there is a collision. This creates a branching of the root node into two child nodes. One with a constraint on the blue robot to avoid the orange robot, and dually for the orange robot (constraints are visualized in red). 
% \ml{shouldn't the constraints be larger and time dependent?}
%\shtodo{Yes, but I think that for brevity we can just say that the constraints prevent both robots from crossing the corridor altogether.}
In both cases, the constraint entirely prevents a valid plan for either agent, although  a-priori a plan does exist.
%Then, when \Alg{CSTR-$\mathcal{X}$} is called to re-plan for the robots, it is likely they that the new trajectories traverse the middle of the corridor again. 
If this behavior is left unresolved, \Alg{K-CBS} would never find a valid plan. Thus, we employ the \emph{merge and restart} technique, borrowed from the discrete setting~\cite{boyarski2015icbs}. Note that in the discrete setting, this is merely a speedup heuristic, whereas for the continuous case it is crucial for completeness.
%This reasoning motivates an additional procedure of \Alg{K-CBS} known as \emph{merge and restart} (MR).
%MR is an improvement of CBS that allows highly coupled robots to be merged into a meta-robot and planned for simultaneously~\cite{boyarski2015icbs}, which we adapt for \Alg{K-CBS}. 
While many merge techniques are available, we utilize a simple, experimentally effective merge policy from~\cite{sharon2012meta}, whereby robots $i$ and $j$ are merged if the number of conflicts between them exceeds some pre-defined threshold $B$. 

The merge policy for \Alg{K-CBS} is shown in Alg.~\ref{alg:K-CBS} (Lines~\ref{ln:mergeIf1}--\ref{ln:mergeIf2} and~\ref{ln:shouldMerge}--\ref{ln:planMeta}). If the \Alg{shouldMerge}() procedure returns true via the requirement above, the two robots are composed together (e.g., Line~\ref{ln:merge}) and another instance of \Alg{K-CBS} is solved for $k-1$ robots where one of the robots in the newly formed problem is a meta-robot (e.g., Line~\ref{ln:solveMeta}). Note that in the case of Fig.~\ref{fig:incomplete}, eventually \Alg{K-CBS} merges the two robots together and plans trajectories that allow both robots to navigate the corridor simultaneously. Also note that we count as conflicts both nodes where a conflict occurs, as well as nodes where no plan is found, via $\mathcal{C}_{\max}$.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Completeness}
\label{sec:completness}
% It is important to note that 
Algorithm
\Alg{K-CBS} inherits the probabilistic completeness property of the underlying Planner $\mathcal{X}$.  
\begin{theorem}[Completeness]
    \label{thm:completeness}
    %If Planner $\mathcal{X}$ is probabilistically complete, then so is \Alg{K-CBS}.
    \Alg{K-CBS} is probabilistically complete if Planner $\mathcal{X}$ is probabilistically complete.
\end{theorem}
\begin{proof}
Ultimately, probabilistic completeness follows from the fact that in the worst case, \Alg{K-CBS} merges all the robots and becomes centralized, and using the completeness of Planner $\mathcal{X}$. 
To show this observe that at each iteration either (1) a merge happens, (2) a conflict node is extended, or (3) a node without a plan receives more planning time. (1) can only happen $k$ times along a branch, (2) can happen at most $k(k-1)B$ times before a merge is made, and (3) happens at most $B$ times for each node. Therefore, in each branch of the tree, eventually either a plan is found or all the agents merge and \Alg{K-CBS} becomes centralized.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Finally, we remark that it may be possible to further improve the performance of \Alg{K-CBS} using heuristics.  Nonetheless, this requires careful treatment and deep understanding of the MRMP problems.  Not every successful heuristic used in MAPF is beneficial in the continuous domain.  For instance, work \cite{boyrasky2015don} shows that, in CBS, significant speedups can be achieved by \emph{bypassing} (BP) a split of a constraint-tree node by generating a single constraint and attempting to resolve it by calling the low-level planner in the same node. Our studies however do not show such improvements by incorporating BP in \Alg{K-CBS}.




% \subsection{Speedup Heuristic: Bypassing Conflicts}
% To further improve the performance of \Alg{K-CBS}, we take inspirations from \cite{boyrasky2015don}.  There, it is shown that splitting a collision into two child-nodes is not always helpful. Rather, it is beneficial to \emph{bypass} (BP) a split by generating a single constraint, and attempting to resolve it by calling the low-level planner in the same constraint-tree node. This essentially prunes the conflict tree, leading to improved performance.
% %prior to splitting in the same constraint-tree node.  %rather, we should simply replace the colliding plan with the new plan. 

% \Alg{K-CBS} with BP is identical to Alg.~\ref{alg:K-CBS} with one key difference in the implementation: when calling \Alg{CSTR-$\mathcal{X}$} for robot $i$, if a trajectory $T_i'$ is found in less than $N$ iterations, the plan corresponding to that node is immediately evaluated for conflicts. If a conflict exists, then we generate a constraint, prune the motion tree $\mathcal{T}$ based on the additional constraint, and then replan again. This process continues until $N$ iterations have been executed -- at which point the most recent trajectory is returned to \Alg{K-CBS}.  
% \ml{Confirm this and modify the following:}
% Our empirical evaluations show that fast computation times can be achieved with the BP heuristic.  The speedup becomes more significant when the number iterations $N$ is large.








==> K-CBS IROS 2022/Sections/Problem.tex <==

Consider $k\in \mathbb{N}$ robotic systems,
in a shared, bounded workspace $W\subseteq \mathbb{R}^d$, $d \in \{2,3\}$, 
which includes a finite set of obstacles $\mathcal{O}$, where every obstacle $o\in \mathcal{O}$ is a closed subset of $W$. Furthermore, every robot $i\in\{1,2,\ldots,k\}$ has a (rigid) body $\mathcal{S}_i$, and its motion is subjected to the following dynamic constraint:
\begin{equation}
    \dot{\mathbf{x}}_i=f_i(\mathbf{x}_i, \mathbf{u}_i), \quad \mathbf{x}_i \in X_i \subseteq \mathbb{R}^{n_i} \quad \mathbf{u}_i=U_i\subseteq\mathbb{R}^{m_i},
    \label{eqn:dyn}
\end{equation}
where $n_i \geq d$, $X_i$ and $U_i$ are robot $i$'s state and input spaces, respectively, and $f_i:X_i\times U_i\rightarrow X_i$ is a continuous and possibly nonlinear function (vector field). With an abuse of notation, we denote by $\mathcal{S}_i(\mathbf{x}_i) \subseteq W$ the set of points that the robot $i$'s body occupies in the workspace when it is at state $\mathbf{x}_i \in X_i$.

Given a time interval $[t_0, t_{fi}]$, where $t_0,t_{fi}\in \mathbb{R}_{\geq 0}$ and $t_0 \leq t_{fi}$, a controller $\mathbf{u}_i:[t_0, t_{fi}]\rightarrow U_i$, 
and initial state $\mathbf{x}_{i,0}\in X_i$ for robot $i$, function $f_i$ can be integrated up to time $t_{fi}$ to form a 
% \emph{trajectory segment} $\mathbf{x}_i^{t_0:t_1}$ for agent $i$, where $\mathbf{x}_i^{t_0:t_1}(t_0)=\mathbf{x}_{i,0}$. 
% Given $\mathbf{x}_{i,0}$, and applying a 
% For $s\in \mathbb{N}$ consecutive controls $u_1,\ldots,u_s$ with respective time intervals
% \begin{equation}
%     [t_0, t_1], [t_1, t_2], \ldots, [t_{s-1}, t_{s}],
% \end{equation}
% we define a 
\emph{trajectory} $T_i:\mathbb{R}_{\geq 0}\rightarrow X_i$ for robot $i$, where $T_i(t_0) = \mathbf{x}_{i,0}$.  
We assume all the robots' trajectories start at time $t_0$.
Further, we assume that, once robot $i$ reaches the end of its trajectory $T_i(t_{fi})$ at time $t_{fi}$, it remains there, i.e., $T_i(t') = T_i(t_{fi})$ for all $t' \geq t_{fi}$.  
% \begin{equation}
    % T_i=\{\mathbf{x}_i^{t_0:t_1}, \mathbf{x}_i^{t_1:t_2}, \ldots, \mathbf{x}_i^{t_{s-1}:t_s}\}
% \end{equation}
% where $\mathbf{x}_i^{t_{l-1}:t_l}(t_l)=\mathbf{x}_i^{t_l:t_{l+1}}(t_l)$ for all $l\in \{1,2,\ldots, s-1\}$, to be a set of $s$ trajectory segments. 
%%%%%%%
Given trajectories  $T_1, T_2, \ldots, T_k$, denote by $t_f = \max \{t_{f1}, t_{f2}, \ldots t_{fk}\}$ the longest time duration of the trajectories.  We say that the trajectories are \emph{collision-free} if the following conditions hold for all $t \in [t_0, t_f]$: 
\begin{enumerate}%[label= (\Roman*)]
    \item $\forall 1\le i\le k$,  $\forall o \in \mathcal{O}$, \quad $\mathcal{S}_i(T_i(t)) \cap o = \emptyset$  \label{cond:obsCollision}
    \item $\forall 1\le i<j\le k$, \qquad \;\;  $\mathcal{S}_i(T_i(t)) \cap \mathcal{S}_j(T_j(t)) = \emptyset$ \label{cond:robotColliision}
\end{enumerate}

%%%%%%%
% Given trajectories  $T_1, T_2, \ldots, T_k$, denote by $t_f = \max \{t_{f1}, t_{f2}, \ldots t_{fk}\}$ the longest time duration of the trajectories.  Then, we say trajectory $T_i$ is \emph{collision-free} if the following conditions hold for all $t \in [t_0, t_f]$: 
% % \begin{align}
% %         \mathcal{S}_i(T_i(t)) &\cap o = \emptyset  \hspace{1.55cm} \forall o \in \mathcal{O}  \label{cond:obsCollision}\\
% %         \mathcal{S}_i(T_i(t)) &\cap \mathcal{S}_j(T_j(t)) = \emptyset \quad  \forall j\in \{1,\ldots,k\}, j \neq i \label{cond:robotColliision}
% % \end{align}
% \begin{enumerate}%[label= (\Roman*)]
%     \item $\mathcal{S}_i(T_i(t)) \cap o = \emptyset$  \hspace{1.4cm} $\forall o \in \mathcal{O}$  \label{cond:obsCollision}
%     \item $\mathcal{S}_i(T_i(t)) \cap \mathcal{S}_j(T_j(t)) = \emptyset$ \quad $\forall j \in \{1,\ldots,k\}, j \neq i$  \label{cond:robotColliision}
% \end{enumerate}
% \shtodo{The quantifiers should come before the condition, unless this is a standard form of writing in robotics.}
% \ml{I thought either way is correct.  But, I'm happy to use a more correct presentation}
% \shtodo{Also, why define collision-free w.r.t. a single trajectory? I think it makes more sense to define w.r.t. the set of trajectories.}
% \ml{ah... I struggled with this one.  I first had it w.r.t to the set of trajectories $T$... but, I had to say for $\forall i \leq k$, the above conditions need to hold, which was hard to read with so many quantifiers.  So, I decided to make it easier to read. If you can find a easy way of presenting it, please go ahead and fix it :)}
\noindent
Condition~\ref{cond:obsCollision} indicates no collision with obstacles, and Condition~\ref{cond:robotColliision} indicates no robot-robot collision.

Given a goal region for every robot, the objective in MRMP is to find a feasible trajectory for every robot to reach its goal without colliding with obstacles nor other robots:
%A formal statement of the problem is as follows. 
% We now define the multi-robot motion planning problem.
\begin{problem}[MRMP]
\label{prob}
% Consider $k$ robotic agents in workspace $W$ with the set of obstacles $\mathcal{O}$.  Given the robot dynamics described in \eqref{eqn:dyn}, initial states $\mathbf{x}_{i,0}, \ldots, \mathbf{x}_{k,0}$, and goal regions $X_1^G, \ldots, X_k^G$, find a controller $\mathbf{u}_i:[t_0, t_{fi}]\rightarrow U_i$ for every $i\in\{1,\ldots, k\}$ such that the obtained trajectory $T_i$ is collision free and takes agent $i$ from $T_i(t_0)=\mathbf{x}_{i,0}$ to $T_i(t_{fi})\in X_i^G$ for every $i\in\{1,\ldots, k\}$.
% while avoiding obstacles $\mathcal{O}$ and all other agents.

Given $k$ robots in workspace $W$ with dynamics as in \eqref{eqn:dyn}, initial states $\mathbf{x}_{i,0} \in X_i$ and goal regions $X_i^G \subseteq X_i$ for all $1\le i\le k$, % \in \{1,\ldots,k\}$, 
find a controller $\mathbf{u}_i:[t_0, t_{fi}]\rightarrow U_i$ for every $1\le i\le k$ such that the induced trajectories $T_1, \ldots, T_k$ are collision-free, and $T_i$ takes agent $i$ from $T_i(t_0)=\mathbf{x}_{i,0}$ to $T_i(t_{fi})\in X_i^G$ for every $1\le i\le k$.
% while avoiding obstacles $\mathcal{O}$ and all other agents.
\end{problem}


==> K-CBS IROS 2022/Sections/table.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{| c | c | c | c | c|} 
%  \hline
%  Number of Agents & Number of Obstacles &  Algorithm & Success Rate (\%) & Mean Computation Time (s)\\ [0.5ex] 
%  \hline\hline
%   10 & 10 & \Alg{pRRT} & 0 & TO\\ 
%  \hline
%   10 & 10 & \Alg{K-CBS} & 92 & 161.7\\ 
%  \hline
%   15 & 10 & \Alg{pRRT} & 0 & TO\\ 
%  \hline
%   15 & 10 & \Alg{K-CBS} & 74 & 226.7\\ 
%  \hline
%  20 & 10 & \Alg{pRRT} & 0 & TO\\
%  \hline
%  20 & 10 & \Alg{K-CBS} & 30 & 290.8\\
%  \hline
%   10 & 5 & \Alg{pRRT} & 0 & TO \\ 
%  \hline
%   10 & 5 & \Alg{K-CBS} & 98.8 & 126.7\\ 
%  \hline
%   15 & 5 & \Alg{pRRT} & 0 & TO \\ 
%  \hline
%   15 & 5 & \Alg{K-CBS} & 92.6 & 203.1 \\ 
%  \hline
%  20 & 5 & \Alg{pRRT} & 0  & TO \\
%  \hline
%  20 & 5 & \Alg{K-CBS} & 0.5 & 279.8\\
%  \hline
%   10 & 0 & \Alg{pRRT} & 0 & TO \\ 
%  \hline
%   10 & 0 & \Alg{K-CBS} & 100 & 104.8 \\ 
%  \hline
%   15 & 0 & \Alg{pRRT} & 0 & TO \\ 
%  \hline
%   15 & 0 & \Alg{K-CBS} & 94.6 & 152.6 \\ 
%  \hline
%  20 & 0 & \Alg{pRRT} & 0 & TO \\
%  \hline
%  20 & 0 & \Alg{K-CBS} & 74.6 & 239.8 \\
%  \hline
% \end{tabular}
% \caption{Benchmark results from variations of $32\times 32$ space.}
% \label{tab:benchmarkTable}
% \end{table*}


% \begin{table*}[t]
% \centering
% \begin{tabular}{| c | c | c | c | c|} 
%  \hline
%  Number of Agents & Number of Obstacles &  \Alg{K-CBS} (succ. rate - comp. time) &  \Alg{pRRT} (succ. rate - comp. time)\\ [0.5ex] 
%  \hline\hline
%   10 & 10 & 92\% - 161.7s & 0\% - TO\\ 
%  \hline
%   15 & 10 & 74\% - 226.7s & 0\% - TO\\ 
%  \hline
%  20 & 10 & 30\% - 290.8s & 0\% - TO\\
%  \hline
%   10 & 5 & 98.8\% - 126.7s & 0\% - TO \\ 
%  \hline
%   15 & 5 & 92.6\% - 203.1s  & 0\% - TO \\ 
%  \hline
%  20 & 5 & 0.5\% - 279.8s & 0\% - TO \\
%  \hline
%   10 & 0 & 100\% - 104.8s & 0\% - TO \\ 
%  \hline
%   15 & 0 & 94.6\% - 152.6s & 0\% - TO \\ 
%  \hline
%  20 & 0 & 74.6\% - 239.8s & 0\% - TO \\
%  \hline
% \end{tabular}
% \caption{Benchmark results from variations of $32\times 32$ space.}
% \label{tab:benchmarkTable}
% \end{table*}

\begin{table}[t]
\caption{Benchmark results for \Alg{K-CBS} in variations of the Large env. (Fig.~\ref{fig:envLarge}). \Alg{pRRT} always timed out.}
\centering
\begin{tabular}{| c | c | c | c | c|} 
 \hline
 \# Agents & \# Obstacles &  succ. rate (\%) & ave. comp. time (s) \\ [0.5ex] 
 \hline\hline
  10 & 10 & 92 & 161.7\\ 
 \hline
  15 & 10 & 74 & 226.7\\ 
 \hline
 20 & 10 & 30 & 290.8\\
 \hline
  10 & 5 & 98 & 126.7\\ 
 \hline
  15 & 5 & 92 & 203.1\\ 
 \hline
 20 & 5 & 50 & 279.8 \\
 \hline
  10 & 0 & 100 & 104.8 \\ 
 \hline
  15 & 0 & 94 & 152.6 \\ 
 \hline
 20 & 0 & 74 & 239.8 \\
 \hline
\end{tabular}
\label{tab:benchmarkTable}
\end{table}
